Human vs Objective Evaluation of Colourisation Performance

Automatic colourisation of grey-scale images is the process of creating a full-colour image from the grey-scale prior. It is an ill-posed problem, as there are many plausible colourisations for a given grey-scale prior. The current SOTA in auto-colourisation involves image-to-image type Deep Convolutional Neural Networks with Generative Adversarial Networks showing the greatest promise. The end goal of colourisation is to produce full colour images that appear plausible to the human viewer, but human assessment is costly and time consuming. This work assesses how well commonly used objective measures correlate with human opinion. We also attempt to determine what facets of colourisation have the most significant effect on human opinion. For each of 20 images from the BSD dataset, we create 65 recolourisations made up of local and global changes. Opinion scores are then crowd sourced using the Amazon Mechanical Turk and together with the images this forms an extensible dataset called the Human Evaluated Colourisation Dataset (HECD). While we find statistically significant correlations between human-opinion scores and a small number of objective measures, the strength of the correlations is low. There is also evidence that human observers are most intolerant to an incorrect hue of naturally occurring objects.

==> Tables/Ground_Truth_GlobalMeanOfChromaMeans.tex <==
\begin{table}
\centering
\caption{Mean zScore after changing all chroma value of Ground Truth  image}
\begin{tabular}{lr}
\toprule
Change Global Mean of Chroma &  Mean z-score \\
\midrule
            Chroma Mean -2sd &        -0.569 \\
            Chroma Mean -1sd &        -0.027 \\
      Ground Truth Reference &         0.364 \\
            Chroma Mean +1sd &         0.124 \\
            Chroma Mean +2sd &        -0.351 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/Ground_Truth_GlobalSpreadOfChromaMeans.tex <==
\begin{table}
\centering
\caption{Mean zScore for changes in contrast of chroma for Ground Truth  images.}
\begin{tabular}{lr}
\toprule
Change Global spread of Chroma &  Mean z-score \\
\midrule
             Chroma 0.25 width &        -0.089 \\
              Chroma 0.5 width &         0.163 \\
        Ground Truth Reference &         0.364 \\
              Chroma 2.0 width &         0.193 \\
              Chroma 4.0 width &        -0.402 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/Ground_Truth_SegmentMeanOfChromaMeans.tex <==
\begin{table}
\centering
\caption{Mean zScores for images with segment changed in chroma for Ground Truth  image.}
\begin{tabular}{lr}
\toprule
Change Segment Mean of Chroma &  Mean z-score \\
\midrule
     Chroma Segment Mean -2sd &         0.061 \\
     Chroma Segment Mean -1sd &         0.184 \\
       Ground Truth Reference &         0.364 \\
     Chroma Segment Mean +1sd &         0.362 \\
     Chroma Segment Mean +2sd &         0.198 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/Ground_Truth_SegmentMeanOfHuesMeans.tex <==
\begin{tabular}{lr}
\toprule
 Change Segment Mean of Hue &  Mean z-score \\
\midrule
   Hue segment shift by -64 &        -0.185 \\
   Hue segment shift by -32 &        -0.020 \\
   Hue segment shift by -16 &         0.268 \\
    Hue segment shift by -8 &         0.373 \\
    Hue segment shift by -4 &         0.367 \\
    Hue segment shift by -2 &         0.369 \\
     Ground Truth Reference &         0.376 \\
    Hue segment shift by +2 &         0.348 \\
    Hue segment shift by +4 &         0.320 \\
    Hue segment shift by +8 &         0.259 \\
   Hue segment shift by +16 &         0.062 \\
   Hue segment shift by +32 &        -0.130 \\
   Hue segment shift by +64 &        -0.227 \\
Hue segment shift by +/-128 &        -0.323 \\
\bottomrule
\end{tabular}


==> Tables/Ground_Truth_Segment_mean_chroma_mann_whit_u_pvalues.tex <==
\begin{table}
\centering
\caption{Mann Whittney U p-values for row is greater than column for changes to chroma of a single segment of Ground Truth  image }
\begin{tabular}{lrrrrr}
\toprule
                         &  \rotatebox{90}{Chroma Mean -2sd} &  \rotatebox{90}{Chroma Mean -1sd} &  \rotatebox{90}{Reference} &  \rotatebox{90}{Chroma Mean +1sd} &  \rotatebox{90}{Chroma Mean +2sd} \\
\midrule
Chroma Segment Mean -2sd &                             0.500 &                             0.961 &                      1.000 &                             1.000 &                             0.970 \\
Chroma Segment Mean -1sd &                             0.039 &                             0.500 &                      1.000 &                             0.999 &                             0.556 \\
               Reference &                             0.000 &                             0.000 &                      0.500 &                             0.837 &                             0.000 \\
Chroma Segment Mean +1sd &                             0.000 &                             0.001 &                      0.164 &                             0.500 &                             0.003 \\
Chroma Segment Mean +2sd &                             0.030 &                             0.445 &                      1.000 &                             0.997 &                             0.500 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/Ground_Truth_Segment_mean_hue_mann_whit_u_pvalues.tex <==
\begin{table}
\centering
\caption{Mann Whitney U test P-values for Ground Truth , where row is greater zScore than column}
\label{HueSegPGround Truth }
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lllllllllllllll}
\toprule
                            & \rotatebox{90}{Hue segment shift by -64} & \rotatebox{90}{Hue segment shift by -32} & \rotatebox{90}{Hue segment shift by -16} & \rotatebox{90}{Hue segment shift by -8} & \rotatebox{90}{Hue segment shift by -4} & \rotatebox{90}{Hue segment shift by -2} & \rotatebox{90}{Reference} & \rotatebox{90}{Hue segment shift by +2} & \rotatebox{90}{Hue segment shift by +4} & \rotatebox{90}{Hue segment shift by +8} & \rotatebox{90}{Hue segment shift by +16} & \rotatebox{90}{Hue segment shift by +32} & \rotatebox{90}{Hue segment shift by +64} & \rotatebox{90}{Hue segment shift by +/-128} \\
\midrule
   Hue segment shift by -64 &                                      0.5 &                                    0.978 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                    0.999 &                                    0.735 &                                     0.25 &                      \colorbox{pink}{0.044} \\
   Hue segment shift by -32 &                   \colorbox{pink}{0.022} &                                      0.5 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                    0.924 &                                     0.08 &                   \colorbox{pink}{0.002} &                        \colorbox{pink}{0.0} \\
   Hue segment shift by -16 &                                      0.5 &                     \colorbox{pink}{0.0} &                                      0.5 &                                   0.956 &                                   0.959 &                                   0.958 &                     0.885 &                                   0.875 &                                   0.769 &                                   0.384 &                   \colorbox{pink}{0.001} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by -8 &                   \colorbox{pink}{0.044} &                     \colorbox{pink}{0.0} &                   \colorbox{pink}{0.044} &                                     0.5 &                                   0.482 &                                   0.446 &                     0.078 &                                   0.234 &                                   0.101 &                  \colorbox{pink}{0.016} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by -4 &                                    0.482 &                     \colorbox{pink}{0.0} &                   \colorbox{pink}{0.042} &                                   0.518 &                                     0.5 &                                   0.487 &    \colorbox{pink}{0.048} &                                   0.272 &                                   0.089 &                  \colorbox{pink}{0.015} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by -2 &                                    0.446 &                     \colorbox{pink}{0.0} &                   \colorbox{pink}{0.042} &                                   0.554 &                                   0.513 &                                     0.5 &    \colorbox{pink}{0.043} &                                   0.266 &                                   0.093 &                  \colorbox{pink}{0.015} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
                  Reference &                                    0.957 &                     \colorbox{pink}{0.0} &                                    0.115 &                                   0.922 &                                   0.952 &                                   0.957 &                       0.5 &                                   0.893 &                                   0.306 &                                   0.063 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by +2 &                                    0.734 &                     \colorbox{pink}{0.0} &                                    0.125 &                                   0.766 &                                   0.728 &                                   0.734 &                     0.107 &                                     0.5 &                                   0.215 &                  \colorbox{pink}{0.049} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by +4 &                                    0.907 &                     \colorbox{pink}{0.0} &                                    0.231 &                                   0.899 &                                   0.911 &                                   0.907 &                     0.694 &                                   0.785 &                                     0.5 &                                   0.157 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by +8 &                                    0.985 &                     \colorbox{pink}{0.0} &                                    0.616 &                                   0.984 &                                   0.986 &                                   0.985 &                     0.937 &                                   0.951 &                                   0.844 &                                     0.5 &                   \colorbox{pink}{0.002} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
   Hue segment shift by +16 &                                      1.0 &                                    0.076 &                                    0.999 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                   0.998 &                                      0.5 &                   \colorbox{pink}{0.003} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
   Hue segment shift by +32 &                                      1.0 &                                     0.92 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                    0.997 &                                      0.5 &                                    0.076 &                      \colorbox{pink}{0.007} \\
   Hue segment shift by +64 &                                      1.0 &                                    0.998 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                    0.924 &                                      0.5 &                                       0.144 \\
Hue segment shift by +/-128 &                                      1.0 &                                      1.0 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                    0.993 &                                    0.856 &                                         0.5 \\
\bottomrule
\end{tabular}}
\end{table}


==> Tables/Natural_Segment_mean_hue_mann_whit_u_pvalues.tex <==
\begin{table}
\centering
\caption{Mann Whitney U test P-values for Natural , where row is greater zScore than column}
\label{HueSegPNatural }
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lllllllllllllll}
\toprule
                            & \rotatebox{90}{Hue segment shift by -64} & \rotatebox{90}{Hue segment shift by -32} & \rotatebox{90}{Hue segment shift by -16} & \rotatebox{90}{Hue segment shift by -8} & \rotatebox{90}{Hue segment shift by -4} & \rotatebox{90}{Hue segment shift by -2} & \rotatebox{90}{Reference} & \rotatebox{90}{Hue segment shift by +2} & \rotatebox{90}{Hue segment shift by +4} & \rotatebox{90}{Hue segment shift by +8} & \rotatebox{90}{Hue segment shift by +16} & \rotatebox{90}{Hue segment shift by +32} & \rotatebox{90}{Hue segment shift by +64} & \rotatebox{90}{Hue segment shift by +/-128} \\
\midrule
   Hue segment shift by -64 &                                      0.5 &                                      1.0 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                     0.99 &                                    0.835 &                                       0.284 \\
   Hue segment shift by -32 &                     \colorbox{pink}{0.0} &                                      0.5 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
   Hue segment shift by -16 &                                      0.5 &                     \colorbox{pink}{0.0} &                                      0.5 &                                   0.969 &                                   0.704 &                                   0.866 &                     0.914 &                                   0.985 &                                   0.822 &                                   0.192 &                                      0.1 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by -8 &                   \colorbox{pink}{0.032} &                     \colorbox{pink}{0.0} &                   \colorbox{pink}{0.032} &                                     0.5 &                                   0.073 &                                   0.192 &                     0.214 &                                   0.561 &                                   0.143 &                  \colorbox{pink}{0.003} &                   \colorbox{pink}{0.001} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by -4 &                                    0.073 &                     \colorbox{pink}{0.0} &                                    0.296 &                                   0.927 &                                     0.5 &                                   0.763 &                     0.804 &                                   0.968 &                                   0.612 &                  \colorbox{pink}{0.043} &                   \colorbox{pink}{0.014} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by -2 &                                    0.192 &                     \colorbox{pink}{0.0} &                                    0.134 &                                   0.808 &                                   0.237 &                                     0.5 &                     0.447 &                                   0.872 &                                   0.356 &                  \colorbox{pink}{0.009} &                   \colorbox{pink}{0.003} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
                  Reference &                                    0.553 &                     \colorbox{pink}{0.0} &                                    0.086 &                                   0.787 &                                   0.197 &                                   0.553 &                       0.5 &                                   0.896 &                                   0.255 &                  \colorbox{pink}{0.003} &                   \colorbox{pink}{0.001} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by +2 &                                    0.128 &                     \colorbox{pink}{0.0} &                   \colorbox{pink}{0.015} &                                    0.44 &                  \colorbox{pink}{0.032} &                                   0.128 &                     0.104 &                                     0.5 &                                   0.056 &                    \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by +4 &                                    0.644 &                     \colorbox{pink}{0.0} &                                    0.178 &                                   0.857 &                                   0.388 &                                   0.644 &                     0.746 &                                   0.944 &                                     0.5 &                  \colorbox{pink}{0.025} &                   \colorbox{pink}{0.007} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by +8 &                                    0.991 &                     \colorbox{pink}{0.0} &                                    0.808 &                                   0.997 &                                   0.957 &                                   0.991 &                     0.997 &                                     1.0 &                                   0.975 &                                     0.5 &                                     0.27 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
   Hue segment shift by +16 &                                    0.997 &                     \colorbox{pink}{0.0} &                                      0.9 &                                   0.999 &                                   0.986 &                                   0.997 &                     0.999 &                                     1.0 &                                   0.993 &                                    0.73 &                                      0.5 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
   Hue segment shift by +32 &                                      1.0 &                                      1.0 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                      0.5 &                                    0.097 &                      \colorbox{pink}{0.002} \\
   Hue segment shift by +64 &                                      1.0 &                                      1.0 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                    0.903 &                                      0.5 &                                       0.065 \\
Hue segment shift by +/-128 &                                      1.0 &                                      1.0 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                    0.998 &                                    0.935 &                                         0.5 \\
\bottomrule
\end{tabular}}
\end{table}


==> Tables/SOTA_mann_whit_u_pvalues.tex <==
\begin{table}
\centering
\caption{P values based on Mann-Whittney-U comparison of row method is better than column method.}
\label{SOTAPVals}
\begin{tabular}{lrrrrrr}
\toprule
          &  DeOldify &  PhotoShop &  Iizuka &  Larsson &  Zhang 1 &  Zhang 2 \\
\midrule
 DeOldify &     0.500 &      0.001 &   0.000 &    0.000 &    0.000 &    0.000 \\
PhotoShop &     0.999 &      0.500 &   0.031 &    0.005 &    0.000 &    0.005 \\
   Iizuka &     1.000 &      0.969 &   0.500 &    0.204 &    0.021 &    0.195 \\
  Larsson &     1.000 &      0.995 &   0.796 &    0.500 &    0.109 &    0.489 \\
  Zhang 1 &     1.000 &      1.000 &   0.979 &    0.891 &    0.500 &    0.887 \\
  Zhang 2 &     1.000 &      0.995 &   0.805 &    0.511 &    0.113 &    0.500 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/Spatial_shift_mann_whit_u_pvalues.tex <==
\begin{table}
\centering
\caption{Mann whitney U p-values for Row is greater than column for spatial shift of colour channels x 1/100 relative to L-Channel}
\label{SpatialP}
\begin{tabular}{lrrrrr}
\toprule
          &  Reference &  Shift 1 &  Shift 2 &  Shift 3 &  Shift 4 \\
\midrule
Reference &        0.5 &      0.0 &      0.0 &      0.0 &      0.0 \\
  Shift 1 &        1.0 &      0.5 &      0.0 &      0.0 &      0.0 \\
  Shift 2 &        1.0 &      1.0 &      0.5 &      0.0 &      0.0 \\
  Shift 3 &        1.0 &      1.0 &      1.0 &      0.5 &      0.0 \\
  Shift 4 &        1.0 &      1.0 &      1.0 &      1.0 &      0.5 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/White_Balance_GlobalMeanOfChromaMeans.tex <==
\begin{table}
\centering
\caption{Mean zScore after changing all chroma value of White Balance  image}
\begin{tabular}{lr}
\toprule
Change Global Mean of Chroma &  Mean z-score \\
\midrule
            Chroma Mean -2sd &        -0.633 \\
            Chroma Mean -1sd &        -0.213 \\
     White Balance Reference &         0.376 \\
            Chroma Mean +1sd &         0.364 \\
            Chroma Mean +2sd &        -0.187 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/White_Balance_GlobalSpreadOfChromaMeans.tex <==
\begin{table}
\centering
\caption{Mean zScore for changes in contrast of chroma for White Balance  images.}
\begin{tabular}{lr}
\toprule
Change Global spread of Chroma &  Mean z-score \\
\midrule
             Chroma 0.25 width &        -0.022 \\
              Chroma 0.5 width &         0.168 \\
       White Balance Reference &         0.376 \\
              Chroma 2.0 width &         0.243 \\
              Chroma 4.0 width &        -0.238 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/White_Balance_Global_width_chroma_mann_whit_u_pvalues.tex <==
\begin{table}
\centering
\caption{Mann whitney U p-values for Row is greater than column for chroma contrast change in White Balance  image}
\label{chromaContrastPWhite Balance }
\begin{tabular}{lrrrrr}
\toprule
                        &  \rotatebox{90}{Chroma 0.25 width} &  \rotatebox{90}{Chroma 0.5 width} &  \rotatebox{90}{Reference} &  \rotatebox{90}{Chroma 2.0 width} &  \rotatebox{90}{Chroma 4.0 width} \\
\midrule
      Chroma 0.25 width &                              0.500 &                             0.998 &                      1.000 &                             1.000 &                               0.0 \\
       Chroma 0.5 width &                              0.002 &                             0.500 &                      0.999 &                             0.817 &                               0.0 \\
White Balance Reference &                              0.000 &                             0.001 &                      0.500 &                             0.037 &                               0.0 \\
       Chroma 2.0 width &                              0.000 &                             0.183 &                      0.963 &                             0.500 &                               0.0 \\
       Chroma 2.0 width &                              1.000 &                             1.000 &                      1.000 &                             1.000 &                               0.5 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/White_Balance_SegmentMeanOfChromaMeans.tex <==
\begin{table}
\centering
\caption{Mean zScores for images with segment changed in chroma for White Balance  image.}
\begin{tabular}{lr}
\toprule
Change Segment Mean of Chroma &  Mean z-score \\
\midrule
     Chroma Segment Mean -2sd &        -0.054 \\
     Chroma Segment Mean -1sd &         0.220 \\
      White Balance Reference &         0.376 \\
     Chroma Segment Mean +1sd &         0.404 \\
     Chroma Segment Mean +2sd &         0.284 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/White_Balance_SegmentMeanOfHuesMeans.tex <==
\begin{tabular}{lr}
\toprule
 Change Segment Mean of Hue &  Mean z-score \\
\midrule
   Hue segment shift by -64 &        -0.248 \\
   Hue segment shift by -32 &         0.025 \\
   Hue segment shift by -16 &         0.188 \\
    Hue segment shift by -8 &         0.324 \\
    Hue segment shift by -4 &         0.292 \\
    Hue segment shift by -2 &         0.428 \\
    White Balance Reference &         0.376 \\
    Hue segment shift by +2 &         0.465 \\
    Hue segment shift by +4 &         0.392 \\
    Hue segment shift by +8 &         0.265 \\
   Hue segment shift by +16 &         0.308 \\
   Hue segment shift by +32 &        -0.010 \\
   Hue segment shift by +64 &        -0.189 \\
Hue segment shift by +/-128 &        -0.243 \\
\bottomrule
\end{tabular}


==> Tables/White_Balance_Segment_mean_chroma_mann_whit_u_pvalues.tex <==
\begin{table}
\centering
\caption{Mann Whittney U p-values for row is greater than column for changes to chroma of a single segment of White Balance  image }
\begin{tabular}{lrrrrr}
\toprule
                         &  \rotatebox{90}{Chroma Mean -2sd} &  \rotatebox{90}{Chroma Mean -1sd} &  \rotatebox{90}{Reference} &  \rotatebox{90}{Chroma Mean +1sd} &  \rotatebox{90}{Chroma Mean +2sd} \\
\midrule
Chroma Segment Mean -2sd &                               0.5 &                             1.000 &                      1.000 &                             1.000 &                             1.000 \\
Chroma Segment Mean -1sd &                               0.0 &                             0.500 &                      0.989 &                             0.995 &                             0.853 \\
               Reference &                               0.0 &                             0.011 &                      0.500 &                             0.679 &                             0.118 \\
Chroma Segment Mean +1sd &                               0.0 &                             0.005 &                      0.321 &                             0.500 &                             0.066 \\
Chroma Segment Mean +2sd &                               0.0 &                             0.147 &                      0.882 &                             0.935 &                             0.500 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/White_Balance_Segment_mean_hue_mann_whit_u_pvalues.tex <==
\begin{table}
\centering
\caption{Mann Whitney U test P-values for White Balance, where row is greater zScore than column}
\label{HueSegPWhite Balance }
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lllllllllllllll}
\toprule
                            & \rotatebox{90}{Hue segment shift by -64} & \rotatebox{90}{Hue segment shift by -32} & \rotatebox{90}{Hue segment shift by -16} & \rotatebox{90}{Hue segment shift by -8} & \rotatebox{90}{Hue segment shift by -4} & \rotatebox{90}{Hue segment shift by -2} & \rotatebox{90}{Reference} & \rotatebox{90}{Hue segment shift by +2} & \rotatebox{90}{Hue segment shift by +4} & \rotatebox{90}{Hue segment shift by +8} & \rotatebox{90}{Hue segment shift by +16} & \rotatebox{90}{Hue segment shift by +32} & \rotatebox{90}{Hue segment shift by +64} & \rotatebox{90}{Hue segment shift by +/-128} \\
\midrule
   Hue segment shift by -64 &                                      0.5 &                                      1.0 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                    0.999 &                                    0.759 &                                       0.563 \\
   Hue segment shift by -32 &                     \colorbox{pink}{0.0} &                                      0.5 &                                     0.98 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                   0.999 &                                      1.0 &                                     0.26 &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
   Hue segment shift by -16 &                                      0.5 &                    \colorbox{pink}{0.02} &                                      0.5 &                                   0.951 &                                   0.923 &                                   0.999 &                     0.993 &                                     1.0 &                                   0.998 &                                    0.82 &                                    0.944 &                   \colorbox{pink}{0.005} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by -8 &                   \colorbox{pink}{0.049} &                     \colorbox{pink}{0.0} &                   \colorbox{pink}{0.049} &                                     0.5 &                                   0.418 &                                   0.928 &                     0.791 &                                   0.985 &                                   0.877 &                                   0.221 &                                    0.446 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by -4 &                                    0.418 &                     \colorbox{pink}{0.0} &                                    0.077 &                                   0.582 &                                     0.5 &                                   0.961 &                     0.866 &                                   0.993 &                                   0.921 &                                   0.236 &                                    0.504 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by -2 &                                    0.928 &                     \colorbox{pink}{0.0} &                   \colorbox{pink}{0.001} &                                   0.072 &                  \colorbox{pink}{0.039} &                                     0.5 &                     0.244 &                                   0.758 &                                   0.356 &                  \colorbox{pink}{0.007} &                   \colorbox{pink}{0.046} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
                  Reference &                                    0.756 &                     \colorbox{pink}{0.0} &                   \colorbox{pink}{0.007} &                                   0.209 &                                   0.134 &                                   0.756 &                       0.5 &                                   0.923 &                                   0.626 &                  \colorbox{pink}{0.029} &                                    0.131 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by +2 &                                    0.242 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                  \colorbox{pink}{0.015} &                  \colorbox{pink}{0.007} &                                   0.242 &                     0.077 &                                     0.5 &                                   0.137 &                  \colorbox{pink}{0.001} &                   \colorbox{pink}{0.007} &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by +4 &                                    0.644 &                     \colorbox{pink}{0.0} &                   \colorbox{pink}{0.002} &                                   0.123 &                                   0.079 &                                   0.644 &                     0.374 &                                   0.863 &                                     0.5 &                  \colorbox{pink}{0.018} &                                    0.079 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
    Hue segment shift by +8 &                                    0.993 &                   \colorbox{pink}{0.001} &                                     0.18 &                                   0.779 &                                   0.764 &                                   0.993 &                     0.971 &                                   0.999 &                                   0.982 &                                     0.5 &                                    0.713 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
   Hue segment shift by +16 &                                    0.954 &                     \colorbox{pink}{0.0} &                                    0.057 &                                   0.554 &                                   0.496 &                                   0.954 &                     0.869 &                                   0.993 &                                   0.921 &                                   0.287 &                                      0.5 &                     \colorbox{pink}{0.0} &                     \colorbox{pink}{0.0} &                        \colorbox{pink}{0.0} \\
   Hue segment shift by +32 &                                      1.0 &                                     0.74 &                                    0.995 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                      0.5 &                   \colorbox{pink}{0.006} &                      \colorbox{pink}{0.001} \\
   Hue segment shift by +64 &                                      1.0 &                                      1.0 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                    0.994 &                                      0.5 &                                       0.292 \\
Hue segment shift by +/-128 &                                      1.0 &                                      1.0 &                                      1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                       1.0 &                                     1.0 &                                     1.0 &                                     1.0 &                                      1.0 &                                    0.999 &                                    0.708 &                                         0.5 \\
\bottomrule
\end{tabular}}
\end{table}

